Navigating the Data Lake with Datamaran: Automatically Extracting Structure from Log Datasets

Organizations routinely accumulate semi-structured log datasets generated as the output of code; these datasets remain unused and uninterpreted, and occupy wasted space - this phenomenon has been colloquially referred to as "data lake" problem. One approach to leverage these semi-structured datasets is to convert them into a structured relational format, following which they can be analyzed in conjunction with other datasets. We present Datamaran, an tool that extracts structure from semi-structured log datasets with no human supervision. Datamaran automatically identifies field and record endpoints, separates the structured parts from the unstructured noise or formatting, and can tease apart multiple structures from within a dataset, in order to efficiently extract structured relational datasets from semi-structured log datasets, at scale with high accuracy. Compared to other unsupervised log dataset extraction tools developed in prior work, Datamaran does not require the record boundaries to be known beforehand, making it much more applicable to the noisy log files that are ubiquitous in data lakes. Datamaran can successfully extract structured information from all datasets used in prior work, and can achieve 95% extraction accuracy on automatically collected log datasets from GitHub - a substantial 66% increase of accuracy compared to unsupervised schemes from prior work. Our user study further demonstrates that the extraction results of Datamaran are closer to the desired structure than competing algorithms.

==> discussion.tex <==
%!TEX root=vldb.tex

\section{Performance Discussion}\label{sec_discussion}

Now that we have described the algorithmic details of \algname,
we are now in a better position to compare the capabilities of \algname
with other tools. 
In Section~\ref{sec_intuition}, we compare the high-level intuition 
of \algname and RecordBreaker~\cite{recordbreaker}
and discuss why \algname's approach is superior. 
In Section~\ref{sec_theory}, we analyze the time complexity of \algname 
and provide a theoretical correctness guarantee.
%In Section~\ref{sec_post_processing}, we describe the structure-refinement techniques that enhance the extraction accuracy of \algname. 

\subsection{Comparison with RecordBreaker}\label{sec_intuition}

In \algname, we adopted a fundamentally different approach 
to RecordBreaker~\cite{recordbreaker}, the unsupervised adaption of 
prior semi-supervised structure extraction systems. 
In this section, we compare the high-level intuition of two systems, 
and discuss why \algname's approach is superior.

\vspace{5pt}
\noindent \textbf{RecordBreaker's Approach.}
The core task of the structure extraction problem is to identify
the correct structure template, 
which is challenging due to the structural uncertainty of record templates 
(see Figure~\ref{fig_record_template_variation} in Section~\ref{sec_problem_definition}). 
RecordBreaker's approach is based on summarization: the program first extracts all record templates, 
then tries to find the best structure template that summarizes all record templates. 
The left hand side of Figure~\ref{fig_approach_flow} illustrates RecordBreaker's approach.

\vspace{5pt}
\noindent \textbf{The Problem with RecordBreaker's Approach.}
Assumption~\ref{ass_boundary} (i.e., the boundaries of records can be identified beforehand) 
is the key assumption in RecordBreaker's approach. 
In order to summarize the common structure from record templates, 
it is necessary that most of the record templates are correctly identified, 
which requires that we know the boundaries of records beforehand.

However, as we will see in our experimental study in Section~\ref{sec_experiment}, 
Assumption~\ref{ass_boundary} doesn't hold for many log files. 
In fact, there are three common characteristics of log files that 
make it nearly impossible to determine the boundaries of records in advance:
\begin{denselist}
\item
\emph{Multi-line}: each record can occupy more than one line. 
\item
\emph{Noise}: a significant fraction of the file are noise.
\item
\emph{Interleaved}: there can be multiple types of records.
\end{denselist}

\begin{figure}[h]
	\vspace{-10pt}
	\begin{center}
		\includegraphics[width = 8cm]{characteristics.png}
	\end{center}
	\vspace{-15pt}
	\caption{Log File Characteristics}\label{fig_log_characteristics}
		\vspace{-10pt}
\end{figure}

Figure~\ref{fig_log_characteristics} illustrates an 
example (fictitious) dataset with all three characteristics, 
for which it is clear that Assumption~\ref{ass_boundary} is false. 
Since RecordBreaker relies on Assumption~\ref{ass_boundary},  
it is impossible for their system to handle such kind of datasets. % Therefore, the main goal of the our algorithmic design in \algname is to extract structure templates directly without first finding all the record templates.

\vspace{5pt}
\noindent \textbf{\algname's Approach.}
In \algname, we adopted a different approach for this task: 
we infer the most plausible structure template directly from each record template. 
We first transform all record templates into structure templates, 
then identify those with sufficient coverage across the dataset. 
The right hand side of Figure~\ref{fig_approach_flow} illustrates \algname's approach. 


Note that \algname's approach no longer requires Assumption~\ref{ass_boundary}: by simply enumerating every pair of nearby \verb|'\n'| characters, we can guarantee that all the correct record boundary pairs are being accounted for. Now, this collection of ``potential records'' contains all the actual records, but it also contains a lot of noise. Therefore, we no longer try to find structure templates that explain all the record templates, but only find structure templates covering a sufficient portion of these ``potential record templates''.

%\subsection{Structure Refinement}\label{sec_post_processing}
%
%The key question regarding the applicability of our approach is whether it is possible to directly extract the optimal structure template from local record templates. During our experimental study, we found that although it is not always possible to extract the correct structure template using only the information from one single record template, in most cases we can find structure templates that are very close to the correct one.
%
%Therefore, we developed two techniques to refine the structures during the evaluation step in order to enhance the applicability of \algname. These techniques attempt to revise the current structure template, and the revised structure templates are then compared against the original ones (using the scoring function or other metrics). We replace the original structure template with the revised ones if necessary.
%
%\vspace{5pt}
%\noindent \textbf{The Array Unfolding Technique} %\slhuang{how and when to use this tech?}
%\vspace{5pt}
%
%During the pruning step, we transform record templates into structure templates by finding the minimum structure template that can generate the record template. However, sometimes the minimum structure template may not be the optimal one. For instance, in comma-separated values (CSV) files, the record template (which looks like \verb|"F,F,F,....,F,F\n"|) should be treated as struct instead of array.
%%\slhuang{after the pruning step, the structure template are minimal. So the final structure templates are also minimal if without Array Unfolding tech.?}
%
%The array unfolding technique is designed to handle this case: for each array-type regular expression in the structure template, we attempt to unfold it by replacing it with a struct-type regular expression. For instance, we can unfold the array-type regular expression \verb|({regex},)*{regex}\n| into struct-type regular expression \verb|{regex},{regex},{regex},{regex}\n|. If the unfolded structure template has better score than the original one, then we can finalize the unfolding.
%
%Partial unfolding is another type of array unfolding mechanism implemented in \algname. In partial unfolding, we attempt to replace the ``first part'' of an array-type regular expression with a struct-type regular expression. For instance, the array-type template \verb|({regex},)*{regex}\n| can be unfolded into the following struct-type template:
%\begin{verbatim}
%{regex},{regex},({regex},)*{regex}\n
%\end{verbatim}
%
%Partial unfolding is primarily used to handle the cases where regular field values are ``mixed up'' with text field values, as in the following example:
%\begin{verbatim}
%Apr 24 04:02:24 srv7 snort shutdown succeeded
%Apr 24 04:02:24 srv7 snort startup succeeded
%Apr 24 14:44:28 srv7 Disabling nightly yum
%\end{verbatim}
%The first four fields are regular fields, but the last one is a free-text field. Note that the minimum structure template here is the single array \verb|(F )*F\n|, but the regular array unfolding technique no longer applies, we have to use the partial unfolding technique to separate these fields apart.
%
%\vspace{5pt}
%\noindent \textbf{The Structure Shifting Technique}
%\vspace{5pt}
%
%\begin{figure}[h]
%	\begin{center}
%		\includegraphics[width = 6cm]{structure_shift.png}
%	\end{center}
%	\vspace{-10pt}
%	\caption{Structure Shifting}\label{fig_structure_shift}
%	\vspace{-10pt}
%\end{figure}
%
%In our experimental study, we found one particular problem with the minimum description length scoring function: it cannot properly distinguish structure templates obtained by cyclic shifting. Figure~\ref{fig_structure_shift} illustrates this phenomenon: the left hand side depicts the correct structure template \verb|LineA\nLineB\nLineC\n|, while the right hand side shows the shifted structure template \verb|LineB\nLine| \verb|C\nLineA\n|. Note that the correct structure template has essentially the same description length as the shifted structure template.
%
%Since it is impossible to distinguish structure shifting using the description length score, another metric is used to compare these shifted structure templates: the position of first occurrence in the dataset. Intuitively, among all the shifted structure templates, the one with the earliest first occurrence is most likely the correct structure.
%


%\subsection{Metadata Description}\label{sec_meta_describe}

%In Section~\ref{sec_evaluation}, there are a lot of metadata in our description length scoring function: for example, the dictionary of enumerated data type, the range for integer data type, etc. Should we include the description length of the metadata in the scoring function? 

%We experimentally studied this question. It turns out that the description length of metadata would make a difference when the dataset size is relatively small. Without metadata description term, the structure templates tend to overfit these small datasets: the algorithm recognizes nearly every field as enumerated type when dataset is small enough. Therefore, we decided to include the description length of all metadata in our scoring function, which seems to have improved the overall extraction accuracy on small datasets.

%\subsection{Other Related Works}

%The problem of finding common structure from a set of records has also been studied in Potter's wheel~\cite{} in a different context. Potter's wheel is a data-cleaning tool, and the structure extraction algorithm is used there to identify the common structure of field values so that outlier can then be automatically identified. The authors developed an exponential time structure extraction algorithm, which works fine for their purpose but not applicable in our setting.

%\todo{We might need to mention DataWrangler as well?}


%Without Assumption~\ref{ass_boundary}, we can no longer know all the instantiated records before we actually know the structure template. Therefore, the top-down approach used in RecordBreaker is no longer applicable. Therefore, we designed the new bottom-up approach in Section~\ref{sec_pruning} to find all structure templates with sufficient coverage.

%Here the intuition is simple: 

%Now we have a collection of ``potential records'' that contains all the actual records but also a lot of noise. In this case, the distributional information will no longer be valid, but the coverage of each structure template is still accurate. Therefore, we can still safely prune out all structure template with less than $\alpha \%$ coverage, as in Algorithm~\ref{alg_pruning}.

%\vspace{5pt}
%\noindent \textbf{The RecordBreaker Approach}
%\vspace{5pt}

% RecordBreaker utilizes a top-down approach to find out the structure template of the dataset: it gathers distributional information of tokens in the record, and then decide whether the top-level symbol is Struct or Array. The same algorithm is applied recursively on each lower-level symbol. 

% The two assumptions above are essential for RecordBreaker's approach to work. However, for many datasets we found in GitHub, these two assumption often do not hold. 
%In the following, we use examples to illustrate these assumptions are not commonly true in log files.

%\vspace{5pt}
%\noindent \textbf{The Problem with Assumption~\ref{ass_boundary}}
%\vspace{5pt}

% There are many log files that consists of more than one type of record. In these kind of datasets, the different types of records are often interleaved arbitrarily, with no obvious rule to tell them part. Figure~\ref{fig_interleave} illustrates this scenario. For this kind of dataset, it would be very difficult for an unsupervised algorithm to detect the boundaries of records.



%\vspace{5pt}
%\noindent \textbf{The Problem with Assumption~\ref{ass_tokenize}}
%\vspace{5pt}

%Assumption~\ref{ass_tokenize} essentially states that there is a predetermined set of characters that can be used to tokenize the records. However, in reality, the set of characters separating field values are often different from datasets to datasets. Here is an example: the comma character \verb|","| is often part of the structure template, but for the following record:
%\begin{verbatim}
%System.TypeLoadException: Could not load 
%type 'PXCMArray<int,4,4>' from assembly ....
%\end{verbatim}
%It would be better if we don't recognize comma as part of the template since the field value \verb|PXCMArray<int,4,4>| contains it.

%\vspace{5pt}
%\noindent \textbf{Our Bottom-Up Approach}
%\vspace{5pt}


==> rebuttal.tex <==
%!TEX root = sigmod2018.tex


\begin{center}
{\LARGE \bf Summary for Revised Paper ``Navigating the Data Lake with {\sc Datamaran}: \\ Automatically Extracting Structure from Log Datasets''}
\end{center}

We thank the reviewers and meta-reviewer for their detailed 
and insightful feedback, and for giving us the opportunity 
to address their feedback in a revision.  
We have prepared a new version of the paper based on their suggestions, 
with updates almost every section, along with a brand new user study section. 
In brief, the changes made include:

%\begin{compactenum}
%\item 
\smallskip
\noindent {\bf \em A. An extensive user study to demonstrate the 
utility of \algname and compare its results 
with that of RecordBreaker.} 
We have performed an extensive user study to understand and quantify the benefits of 
\algname for extraction from 
noisy log datasets, relative to unsupervised structure extraction tools, from a user-centric perspective.  
%provide more meaningful insights on the utility of unsupervised structure extraction tools and why \algname is better tailored towards noisy log datasets. 
A brief summary of the user study can be found in Section~\ref{sec_user_study}, 
with additional technical details in the appendix and the technical report. 

\smallskip
\noindent {\bf \em B. Clarifying the output format and the importance of recognizing multi-line records.} 
We have added a paragraph (with an example---Figure~\ref{fig_relational_format}) 
in Section~\ref{sec_ass_form} to clarify the final output relational format of \algname. 
We have expanded one example in the introduction into two (both with real log datasets)
to explain why recognizing multi-line records is crucial---we also contrast this with
the approach adopted by a line-by-line extraction scheme.

\smallskip
\noindent {\bf \em C. Positioning against several lines of related work 
and eliminating missing references.} 
We have added text in our related work sections to describe the differences between our work and existing
work in structure identification in security research and natural language processing,
as well as log clustering from the data mining literature.

\smallskip
\noindent {\bf \em D. Explaining the algorithmic challenges in \algname.}
To explain what are the concrete technical challenges that \algname has been designed to address,
we added a discussion on the algorithmic challenges and contributions in Section~\ref{sec_alg}.

\smallskip
\noindent {\bf \em E. Other significant writing changes.} 
We have made considerable changes to the text of the paper to improve its overall readability. 
Specifically, we have focused on making the paper more clear, formal, and concise. 
Finally, we have also improved presentation by replotting figures, 
making our notation consistent, and fixing typographical errors.

\smallskip
The changes in the paper are highlighted in \new{\bf blue}. Unfortunately,
due to the new additions, this meant that our paper ended up being longer than we could fit in the 12+4 pages;
additional details  can be found in our extended technical report~\cite{DatamaranTechReport}.
%\end{compactenum}
We address the specific points raised in each of the individual reviews below, starting with the meta-review.

\subsection*{Metareview}
\com{(M1) There is significant work in this area, although much of it comes from other fields. It's important to position the proposed approach against these papers, even though the application may be different.}

We have added text in Section~\ref{sec:related} and Section~\ref{app_related} to summarize 
the differences between structure extraction 
from log datasets and from other types of media, in addition to describing all other references
provided by the reviewers.  

Broadly speaking, these algorithms crucially rely on certain characteristics
that are specific to the extraction target in the application area.
For example, in security research, 
network traces consist of multiple parallel sessions,
separated by IP addresses, where each session corresponds to a continuous communication
between a server and a client. Here, the source/destination IP address is a clear indication 
of which session the message belongs to. The challenge of structure extraction 
in that setting depends on whether the protocol 
is binary or text-formatted, and the consequent strategy 
also differs. In the case of text-formatted protocols (which is more relevant to our paper), 
the record boundaries are clear (i.e., one network packet corresponds to one record), but the 
challenge unique to their setting is that message template depends on the current state of the session
(e.g., the template of the server response depends on the previous client message). 
The papers reviewers
deemed as potentially relevant can also be categorized as described above: 
Whalen et al.~\cite{whalen2010hidden} focuses on 
binary-formatted protocols and uses a Hidden Markov Model, while
Wang et al.~\cite{wang2012semantics} focuses on text-formatted protocols 
and uses a clustering-alignment based two-step approach, 
which relies on the fact that record boundaries 
are already known in network traces. 
Another paper from Wang et al.\cite{wang2011inferring} focuses on 
binary protocols and once again 
attempts to infer the global state machine of the protocol. 
Bossert et al.'s work~\cite{bossert2014towards} focuses on text-formatted protocols 
and also follows the same two-step approach of Wang et al.'s work~\cite{wang2012semantics} 
but with small changes in both the clustering and alignment algorithms to improve performance.
Thus, the primary challenges addressed in this line of work are very different,
and their techniques do not apply to noisy log datasets with unknown record boundaries.

As another example, natural language processing (NLP) structures are usually restricted to 
local context (i.e., within each sentence)---thus, the existence of a period (.) is a clear
separation between ``records'' that need to be extracted independent of each other---and 
are usually captured using probabilistic language models (e.g., hidden markov models or probabilistic context-free grammars). 
Most NLP structure learning papers is therefore about defining better probabilistic language models 
or finding better parameter estimation methods. 
With regards to the references provided by the reviewers on unsupervised structure learning in NLP, 
Cohen et al.'s work~\cite{Cohen2011} first trains the parameters 
of a probabilistic language model on multiple ``helper'' languages with annotated data, 
then restricts the parameter space for the unknown language to 
be within the convex hull of the parameters of all the ``helper'' languages 
to improve the performance of unsupervised structure prediction. 
Spitkovsky et al.~\cite{Spitkovsky2011} investigates 
the possibility of using unsupervised word clustering-based  
labels (based on local neighborhood of words) to train existing supervised algorithms. 
Due to the lack of supervision in the form of helper languages, or 
the fact that utilizing the local neighborhood of words to understand how they are 
used---especially when the field values may often never be repeated in log dataset---is not relevant,
and finally, because record boundaries are not available,
these techniques are inapplicable to log files. 
% These papers are not very relevant to our work because most language models are usually restricted to natural languages.

In our case, the fundamental characteristics of log datasets are captured in Definition~\ref{def_dataset}, 
and our whole extraction strategy revolves around this definition. Raza and Gulwani's work~\cite{raza2017automated} studies the possibility of designing ``generic'' structure extraction algorithms by pushing all problem-specific properties into the design of domain-specific language (DSL). By using the text extraction DSL, their algorithm can theoretically 
be applied to log datasets. However, their approach is still example-based, in the sense that the input to the algorithm needs to be a list of example records. Therefore, they are essentially making the same assumption as in LearnPADS~\cite{fisher2008dirt}, i.e.,  that the log dataset is chunked beforehand. As we have stated in the paper, this is a problematic assumption in practical log datasets containing multi-line records and noise. We do compare against RecordBreaker, an unsupervised adaptation of LearnPADS via both performance experiments and a user study.

Another line of related work in the field of data mining addresses the problem of clustering event log records~\cite{makanju2009clustering, vaarandi2004breadth}.  
In the case of event logs, the record boundaries are clear because of 
the existence of a timestamp, but there are usually many different types of events 
in this type of a log file. 
Makanju et al.~\cite{makanju2009clustering}'s tool IPLoM uses several features for clustering
these records,
such as token count/token position/token bijection: this is, in a sense, a coarse form
of single-line unsupervised extraction, taking into account domain knowlege (i.e., that these features matter for clustering events).
Vaarandi~\cite{vaarandi2004breadth} studied the same problem but used a frequent pattern mining technique.
Among these two tools, only IPLoM attempted to also extract field values 
from records, and by doing so they need to make the strong assumption 
that records of the same type have the same number of tokens. 
Because of these reasons, these algorithms do not work on generic log datasets. 

\com{(M2) The formal properties of the template language were not fully explored, which would help distinguish this work from prior work}

The scope of our template language is formally defined in Assumption~\ref{ass_form}. 
We choose not to fully explore the properties of such a template language because  
it is very similar to the template language in LearnPADS~\cite{fisher2008dirt} 
(we have clarified this in Section~\ref{sec_ass_form}). 
The primary difference is that that we do not use
a union type-construct. However, compared to LearnPADS, 
our definition of a log dataset in Definition~\ref{def_dataset} and the corresponding problem formulation is novel: 
in Definition~\ref{def_dataset}, we defined a log dataset as concatenation of instantiations of multiple types of 
structure templates, plus potentially heavy noise. In contrast, LearnPADS assumes the log dataset to be a well-defined
list of chunked records. As described in the paper, a key difference here is that we no longer assume that record 
boundaries are known beforehand. This difference leads to a very different algorithmic solution.

Moreover, our primary contribution is  more on the algorithmic 
aspects of detecting structure using this template
language rather than template language design.

\com{(M3) There was some concern of incremental results, but also some debate. LearnPADS is ``almost'' unsupervised, in that one only need to provide record boundaries. So the difference could be perceived as small.}

Our paper argues that identifying record boundaries is a major challenge
in noisy log datasets. 
The presence of heavy noise and the existence of multiple types of records 
with different record spans altogether makes it very difficult for users 
to specify all of the possible record boundaries in such datasets (at the very least, they may need to manually write a chunking script). 
Therefore, LearnPADS is not very practical for noisy log datasets. 
We have added text to the introduction, along with real examples, to emphasize this aspect. 
To study this further, we evaluate the amount of supervision necessary
to extract a target structure from the extraction result of the 
unsupervised version of LearnPADS, i.e., RecordBreaker, 
the extraction result of \algname,
as well as the raw file directly via a new user study in Section~\ref{sec_user_study}.
Our user study demonstrates that \algname's results are very close to desired target structures already,
with only minor changes necessary (e.g., deleting unnecessary columns) to reach the eventual target.
Unfortunately, both wrangling the file directly using Excel functionalities,
or starting from the results of RecordBreaker require considerable effort, and are often prone to failure.

\com{(M4) There was concern about the evaluation metric, which was hard to interpret in practice. Simply asking users whether the discovered template is correct would provide a more compelling result, at least for some datasets. ... Better motivate why asking users to validate the template would not be a far more compelling result -- it seems like a "missing" experiment. (Better yet, it would be extremely helpful to add such an experiment, though we stopped short of requiring this.) Related: Explain in more detail why it is infeasible to ask users for examples to provide some supervision?
}

We have rewritten the evaluation metric description to 
clarify some misunderstandings in the reviewer's comments. 
At the same time, we agree that a user study would provide a more compelling result,
but asking the users directly if the structure is correct or not is not straightforward (e.g., what does it mean
for a structure to be ``correct''? what do they compare it to?)
So, to evaluate this, we conducted a user study wherein we asked participants to extract a desired target from the
results of \algname, RecordBreaker, and the raw file, using existing data wrangling functionalities in Microsoft Excel,
such as FlashFill. (We educated all participants on the appropriate functionalities provided by Excel, if needed.)
While our existing metrics support the thesis that \algname can correctly extract all
relevant information, our user study demonstrates why it is better for users
to start with the results of unsupervised extaction results first (so that the user can perform refinement if needed) 
as opposed to asking users to extract from scratch using example-based supervision on the raw file (say, with functionalities like FlashFill). Details can be found in Section~\ref{sec_user_study}.

Regarding the infeasibility of supervision, our claim is the following: {\em given the number of noisy log datasets present
in enterprise data lakes, supervision to extract from each of the 100s of thousands of datasets
is simply impossible}. 
Unsupervised techniques provide a suitable proxy to allow these datasets to be extracted and managed. 
Subsequently, keyword search, data integration, and data analysis, all become easier when the relevant record information
is extracted and the relationships between record attributes is explicitly maintained. 
On the other hand, for data analysis of a specific dataset, supervision is, in fact, absolutely necessary---only the
data analyst knows which fields in a dataset are relevant to a specific analysis task, given that the analyst understands the context 
and the semantics underlying these fields. 
That said, what our user study shows is that even for this form of data analysis, 
starting from the results of \algname is preferable to that of RecordBreaker or the raw file,
since the supervision is a lot less substantial, and less prone to error. 

%We have done our best to implement all the individual reviewer suggestions, and have provided explanations for the few that we are unable to implement. Detailed line-by-line responses follow below.



\subsection*{Reviewer 1}
\com{(A1) 
If we treat each line separately, we can extract the line templates, and then merge templates that always appear consecutively in post-processing. This would likely decrease the search space and potentially speed up this step.}

We agree with the reviewer that it is technically possible to treat each line separately at first, 
and then merge them in post-processing. 
However, in our opinion, this approach is simply delaying the 
difficult part of the problem (i.e., identifying the record boundaries). 
Even with all of the individual lines in the log dataset properly categorized, 
it is still not straightforward as how to merge these lines---the best approach 
that we can think of is to utilize a similar procedure as in the generation step: 
enumerate record boundaries and insert them into a hash-table-like structure to find repeated ones. 
Even from that point on, finding the best multi-line record composition still requires evaluating 
the regularity score function, which is very similar to the evaluation step in \algname. 
Therefore, the two-step approach that the reviewer alludes to will essentially end up with
us having to iterate through the steps in \algname two times. 

In addition, the accuracy of the two-step approach will heavily 
depend on the quality of extraction results in the first step: 
as we have seen in most multi-step data processing pipelines, 
the later steps will amplify all of the mistakes in first few steps.

Finally, a line-by-line extraction mechanism (even if perfect), can
lose information corresponding to the association between the lines that together
constitute a record, especially when multiple types of records exist along with
noise. We have added an example to the introduction to illustrate this. 

Also see our response to comment M2 by the Metareviewer. 

\com{(A2) 
I am unclear on what the final output of the system looks like. 
The abstract and introduction state that the objective is to convert 
logs into structured relational format. What do these relations look like in the end?}

We thank the reviewer for pointing out this omission. 
We have added examples to illustrate the alternative representations for
the output of \algname in Section~\ref{sec_ass_form} 
to show how to convert the extracted results into a relational format.

\com{(A3) The paper focuses on processing complete log files, rather than logs that continue to be appended ...  it would be nice to understand whether these techniques are applicable at all in a continuously growing log.
}

We agree that this is an interesting extension. 
From the perspective of our paper, since we are focused on extracting structure, 
and especially employing sampling to do so (Section~\ref{sec_generation}),
we will not be impacted by the growth of the log dataset, except when it comes to parsing 
the dataset with the structure that has been determined. 


\com{(A4) Finally, a few smaller points that could benefit from some additional clarity:
\begin{denselist}
\item Definition 2.2 discusses field values, but does not mention anything explicitly about data types. Do data types play any role in matching records and templates?
\item Is the main objective of the assumption in 3.2 efficiency? I am not sure I fully understand the necessity of this assumption.
\item In step 2 in Sec 4.1, why do the pairs need to be close to each other?
\item The beginning of Sec 5 provides the default values of the parameters in the evaluation. How are those determined? Are they dataset-speficic?
\end{denselist}}
1. Data type does not play any role in our algorithm (since \algname separates fields purely from delimiters). 
Data type information is only potentially infered and utilized in the \scoreF.

2. Assumption~\ref{ass_main} plays a key role in the generation step: because of this assumption, we can first enumerate 
various values for RT-CharSet, then use these values to separate the fields and formatting characters (delimiters) 
for each individual record. We added some text to clarify this point in Section~\ref{sec_generation}.

3. This is for efficiency. If we enumerate all possible pairs, the time complexity would be quadratic in the dataset size.

4. The default values of the parameters were picked manually based on our intuition 
at the beginning of the experiment, 
and we have used the same parameter settings for most of our 
experiments. In any case, we have additionally experimentally illustrated that 
Datamaran is robust with respect to parameter choices, and, in fact, 
the default parameter setting is not the optimal 
configuration according to our later experiments; parameter variation experiments can be found in our technical report. 

\subsection*{Reviewer 2}
\com{(B1)
Compared to prior work, the main innovation of Datamaran is its ability to recover structure in an unsupervised manner. Beyond that, however, the algorithm used by Datamaran is basically the same as in prior work. }

The main innovation of \algname is the ability to handle multi-line records 
gracefully for noisy log datasets. 
Prior work, such as RecordBreaker or Flashfill require that record boundaries 
are known beforehand, which is not true for noisy log datasets. 
Specifying the record boundaries in noisy log datasets is difficult to do manually
(see Example 2)---in particular, with the large number of datasets in enterprise data
lakes, one cannot expect minute supervision for each dataset. 
The fact that we no longer know the record boundaries
introduces a number of new technical challenges to the problem,
and prior algorithms are no longer applicable. 
In particular,
prior algorithms rely on gathering statistics of and summarizing the patterns obtained at the record level:
this is only possible when record boundaries are known. 
We have now added a discussion to Section~\ref{sec_alg} discussing the major algorithmic
challenges and contributions of \algname. 


\com{(B2)
But the present work is weaker than prior work in that there is no formal grammar for the structure of the templates (are they just regular expressions or something similar to PADS?). }

We formally described the structure of templates in Section~\ref{sec_assumption}. 
Specifically, Assumption~\ref{ass_form} restricts the form that each structure template could take, 
which is similar to the restrictions employed by LearnPADS. See also our response to comment M2 from the Metareviewer.

We also have changed the writing in Section~\ref{sec_alg} 
to make the presence of Assumption~\ref{ass_form} clearer.

\com{(B3)
There is also no guarantee of completeness of the search process, and no refinement mechanism in case where the selected template returned to the user is not what she intended. }

The search procedure is complete in the generation step, 
and we have added one paragraph explaining this aspect in Section~\ref{sec_alg}. 
As for the refinement mechanism, we did not implement any since \algname is not meant to be 
an interactive system, 
and the goal is to primarily aid extraction 
from large enterprise data lakes, allowing these datasets to be used within data integration and keyword search applications. 
However, as the output of \algname is in a relational format (see also our response to comment A2), 
it is possible to use existing data wrangling tool to further refine the result, if needed. 
For example, users could eliminate attributes that they are not interested in analyzing presently. 
This is illustrated in our new user study in Section~\ref{sec_user_study};
our study also demonstrates that it actually takes less effort to 
refine the extracted results from \algname 
compared to doing it from scratch using example-based supervision.
See also our response to comment M3 from the Metareviewer. 


\com{(B4) If the end user is allowed to provide feedback (e.g., by providing examples) the resulting tool will not need to be so dependent on such ``black-box'' scoring functions. So this makes me wonder whether the unsupervision aspect is worthwhile, especially given the success of FlashFill where desired outputs are solicited from users.
}

For the setting we target---enterprise data lake extraction---it is impossible to use supervision
at scale, especially for 100s of thousands of datasets.
For such settings an unsupervised approach is the {\em only} option.
That said, we believe that unsupervised techniques are valuable, even in the face
of supervised techniques like FlashFill.
Our user study demonstrates this as well.
In particular, we find that the output of \algname is much closer to desired extraction results,
requires much less effort, and is much less error-prone than employing supervision on the raw file,
or on the output of RecordBreaker, especially when employing data wrangling techniques like FlashFill. 
See also our response to comments M3 and M4 from the Metareviewer. 

%This usefulness of unsupervised extraction is also motivated 
%in the work by Raza and Gulwani~\cite{raza2017automated}, 
%who is also the author of FlashFill paper (we now also cite this paper in our related work). 
%We quote ``\textit{PBE approaches depend on an explicit intent specification from the user about the task that they want to perform, which often requires the user to correctly understand the examples that will help the system to infer the correct program, and can also require significant manual effort from the user in many kinds of tasks.}''.

\com{(B5)
I find it very unsatisfactory for the evaluation criteria to be simply all intended extraction targets can be reconstructed by concatenation of fields. As in prior work, the authors should run a user study to confirm that what they have extracted are indeed what the users have in mind (or at least they would find it useful for subsequent task (such as search, as the authors mentioned in the introduction). }

Evaluating an unsupervised extraction tool via a user study is hard to do in general,
since it depends on the specific task that the user has in mind. 
For example, if the user is only interested in the first attribute of the record for the purpose
of their analysis, all tools
that extract the remaining attributes are technically ``incorrect''.
Indeed, most related work in this space did not perform any user study for the purpose of evaluation. 
% Indeed, two major related works (LearnPADS, and Raza \& Gulwani 2017), \blue{the only unsupervised log dataset extraction system that we have seen}, did not perform any use study for evaluation purpose. 
Nevertheless, we added a user study to evaluate whether our system provides a valuable starting point
for analysis, as compared to RecordBreaker or the raw file directly, in Section~\ref{sec_user_study}.
Also see our response to comment M4 from the Metareviewer. 

We remark that coming up with a meaningful and subjective 
evaluation metric is hard for unsupervised extraction tools:  
LearnPADS~\cite{fisher2008dirt} only reported ``extraction accuracy'', 
which is actually hard to be defined objectively. 
In our case, we only consider the extraction 
	to be successful if there exists a series of tabular operations (e.g., 
	concatenating or removing columns) such that after performing these operations 
	all tuples in the extracted tabular dataset will have the ``golden standard 
	structure'', which is actually a very strong condition. To better clarify the 
	rationale behind the scoring function and provide more intuition, we have 
	expanded the evaluation metric description.

\subsection*{Reviewer 3}
\com{(C1)
This work addresses this problem, and in addition studies problem \#2: across multiple lines, how to identify repeating line patterns as potential records. It is not clear under what scenarios is \#2 useful, as it could not seem to directly benefit use cases like data search. It would also be good to discuss what new developments in data or application scenarios make \#2 important. }

We have added one example in our introduction 
to illustrate why it is important to identify multi-line records 
as is, instead of treating them as a union of single-line records. 
Briefly, by treating multi-line records as the union of single-line records, 
the associations between records are completely lost, 
making it hard to reconstruct them for the purpose
of keyword search or data integration. 
This gets especially complicated when there are multiple types of records or noise present in the dataset.
Also see our response to comment M2 by the Metareviewer.

Furthermore, this loss of information could be very problematic, even when attempting to use line-by-line results for analysis, 
as demonstrated in our new user study in Section~\ref{sec_user_study}. In particular,
it is much easier and less error-prone to use \algname's results as opposed to the
results from RecordBreaker to get to a desired target structure. 

\com{(C2)
A side comment here is that the definition of ``records'' can be ambiguous and subjective. For example in the example in Figure 1, A1 and B1 can be considered as one record (for an end-to-end copy operation) instead of two separate ones as suggested by the authors. It seems hard to determine objectively which definition of records among the two is better. }

In most practical log datasets, the best definition of ``records'' is usually relatively straightforward. 
For the example in Figure~\ref{fig_sample_file} (old Figure 1), 
considering AB as one record is not appropriate  
because the order of A and B may be arbitrary in the 
rest of the file (i.e., it could be like ABABBAA, as in our example). 
Considering ``AB'' as a single record is likely a bad idea since 
it will have very little coverage (and is also unintuitive). 
We have modified Figure~\ref{fig_sample_file} to clarify this point.

\com{(C3) Another assumptions made by the authors is that Regex is needed to represent patterns. Prior work only differentiates between constant-strings vs. variable-fields since log records are essentially generated by printf statements that follow strict patterns (printf strings are not generated from Regex). It would be useful to discuss how much additional benefits Regex would bring to the table through an experimental comparison (Regex is more costly to extract and more likely to be incorrect).}

The complicated form of Regex (Assumption~\ref{ass_form}) is necessary in our paper to alleviate the restrictive non-overlapping assumption (Assumption 2). For instance, if white space character ` ' is considered as a delimiter, then all of the free-text fields would be tokenized into several consecutive words (separated by space), and it is necessary to use array-type structure to capture the notion that these tokens belong to the same field. 
Note that our template language in Assumption~\ref{ass_form} is basically the same as in LearnPADS~\cite{fisher2008dirt},
except that we do not use a union type-construct.  
% However, compared to LearnPADS, our definition of log dataset in 
% Definition~\ref{def_dataset} and 
% the corresponding problem formulation is novel: in Definition~\ref{def_dataset},
% we defined the log dataset as concatenation of 
% instantiations of multiple-types of structure templates plus potentially
% heavy noise. In contrast, LearnPADS assumes the log dataset 
% to be a list of records that are chunked beforehand. 
% Thus, the key 
% difference is that we no longer assume record boundaries are known beforehand---this difference
% basically ensures that our algorithm design problem is very different. 

%\agp{Can we state that LearnPADS uses similar restrictions and therefore we aren't reinventing the wheel here?}

We agree that if we do not make Assumption 2, then the form of structure templates can be much simpler. However, in such a case, the formatting characters could also appear within field values, which raises a different type of difficulty for extraction, and our algorithmic framework won't work in such a scenario. 

\com{(C4-C5)
The way accuracy is defined in experiments is a bit convoluted and would seem to favor fine-grained splitting of fields. In particular, a naive approach of grouping highly similar lines together (without considering coverage) and outputting pretty much everything as variable-fields would seem to score very high for example. Would evaluations used in [1] [2] be more straightforward and objective? \ldots 
The authors emphasize that extracting multi-line record patterns is a distinguishing feature of the paper. However that does not seem to be accounted for in the current evaluation setup. A single-line pattern discovery system would seem to score just as well using the proposed metric. Designing a good metric for multi-line records is not straightforward since they are highly subjective as discussed above.}

The accuracy is defined in such a way that if either the record boundaries or the type of record is incorrectly identified, then the extraction result will not be counted as successful. We admit that this point was not very clear from the main paper (it can only be seen from the appendix), and we have rewritten the description of evaluation metric to emphasize this. 

The metric in \cite{vaarandi2004breadth,makanju2009clustering} ([1][2] in the reviewer response) only evaluates whether the records are correctly categorized. However since our work also identifies the structure within each type of records, the metric in \cite{vaarandi2004breadth,makanju2009clustering} ([1][2] in reviewer response) is not sufficient (their condition is actually a prerequisite for our extraction to be viewed as successful). Evaluating the correctness of field identification is not easy (as explained in Section 5.1), and our metric is designed to only penalize coarse-grained splitting (e.g., treating the whole record as a single field). We remark that for the extraction result to be counted as successful, the extracted fields must be well aligned (i.e., there exists a well-defined schema for the extracted relational dataset, see appendix for more details on this aspect), which is more difficult to achieve for fine-grained splitting. We have rewritten the evaluation metric description to clarify these aspects. Nevertheless, the ultimate proof is the user study, where \algname demonstrates a substantial advantage over RecordBreaker in terms of the extraction results.

%\agp{State something like: nevertheless, the ultimate proof is the user study, where we show that we are awesome.}

\com{(C6)
For the experiments in Section 5.2 on manually collected datasets, accuracy is not currently reported for RecordBreaker. }

Most of the manually collected datasets are originally used in the LearnPADS paper, so the point here is that we can perform as well as RecordBreaker on their hand-picked datasets (we trust their tool can extract their hand-picked datasets successfully). The formal comparison is conducted on randomly collected log datasets to ensure fair comparison. 



\com{(C7) The authors propose an ``assimilation score'' to approximate the final ``regularity score''. The design of the approximation score is a bit ad-hoc and can be better justified. }

The entirely of Section 4.2 is dedicated for justifying the ``assimilation score''---we provide many
reasons as well as intuition for why we designed it in that manner. 



